A 2D pixelated stilbene scintillator detector array for simultaneous radiography with fast neutrons and gammas

For radiography applications using fast neutrons simultaneously with gammas we have developed a detector with 16 stilbene crystals in a 4$\times$4 2D array with a 5~mm pitch and a depth of 25~mm. The crystal array is read out by Silicon photomultipliers and custom signal processing electronics. The detector prototype was tested using a custom D-D fast neutron generator at the Paul Scherrer Institute. By applying a pulse shape discrimination algorithm the detector is able to detect and distinguish fast neutrons and gammas simultaneously. Various attenuating samples placed between the source and detector with different materials and thicknesses were tested and the measured macroscopic fast neutron cross sections were compared to what was expected. Deviations were studied with the help of detailed Geant4 simulations. The detection efficiency for D-D fast neutrons was measured to be around 10\%.

==> conclusion.tex <==
The 16 pixel detector prototype presented in this paper was successfully tested with a D-D neutron generator with mean emission energies between approximately 2.3 and 2.8 MeV.  The detector's scintillation material stilbene allows neutron-gamma separation using pulse shape discrimination techniques. Applying these techniques, a neutron detection efficiency, averaged over all pixels, between $(9.11\pm 0.11) \%$ and $(11.95 \pm 0.12) \%$ was determined, applying a conservative lower energy cut by requiring $FOM>1.27$. A higher detection efficiency would be achievable by requiring a less conservative $FOM$ criterion with the disadvantage of a (slightly) larger contamination e.g. of neutron counts by gamma events and difficulties in the comparison with simulations, as neutron events need to be filtered if they lie in a region where they are mixed up with gamma events. This would be interesting if the measurement time needs to be reduced or a weaker neutron source shall be used. 
The detection efficiency was determined for three different angles relative to the generator's ion beam direction, i.e. three different mean neutron energies. Here, it was seen that the efficiency in \SI{90}{\degree} direction was larger than in the \SI{0}{\degree} direction,  which is an unexpected result. Further studies should be done to explain this discrepancy.\\ 
With radiographic attenuation measurements of three different objects, it was shown that the detector setup allows distinguishing different materials and also the presence of material thickness differences of only \SI{0.5}{cm} for measurement times of approximately \SI{0.5}{h} to \SI{1}{h} by calculating a differential rate between measurements with and without object. The accuracy could possibly be improved by increasing the measurement time.  However, if material and thickness would be unknown, in this radiographic measurement approach it would be impossible to accurately identify simultaneously unknown material composition and thickness as there would be too many free variables. \\
From the differential rates, the macroscopic cross section for the attenuators' materials was calculated, showing a systematic underestimation compared to literature values. By using detailed Geant4 simulations, two main contributions for these deviations were identified: Neutrons that interact in the attenuator but still arrive at the detector and multiple interactions in different detector pixels or in the detector box and then in a pixel. Additionally, a possible misalignment of the step wedge was investigated by comparing the simulated and the measured macroscopic cross section values.  It would be interesting to further study the effect of multiple interactions on the determined cross section using the simulations.\\

\noindent In the future, it is planned to further test the potential of the detector concept focusing on two aspects. First, neutron and gamma radiographic images of test objects shall be taken simultaneously, using different neutron sources, e.g. an Americium-Beryllium (AmBe) source. First measurements of this type were done during a master thesis \cite{thesis_christoph} in our group. Second, the potential of taking simultaneous neutron and gamma tomographic images shall be investigated based on the detector concept of a PSD capable solid scintillator such as stilbene coupled to SiPMs. These studies shall be done using Geant4 simulations and test measurements mainly with an AmBe source. A test stand allowing both types of measurements to be performed simultaneously is currently under development. It is also planned to test the capability of combining our detector concept with a HPGe detector for Neutron Activation Analyses.


==> detector.tex <==
\subsection{The $4\times4$ pixel detector}
The detector consists of 16 stilbene scintillator cuboids that are arranged in a $4 \times 4$ array allowing the detection of neutrons and gammas with spatial resolution. The scintillators are cuboids of size $5 \times 5 \times 25\,\mathrm{mm^3}$ and are coupled to a Hamamatsu MPPC\textsuperscript{\textregistered} S13361-6050AE-04 SiPM array \cite{sipmarray}. The cuboids are separated by a grid made from black PVC\footnote{Polyvinyl chloride}. Everything is surrounded by a black PVC housing to shield it from ambient light. All PVC surfaces facing the scintillators are covered by Vikuiti{\texttrademark} ESR (Enhanced Specular Reflecting) foil to enhance the light collection efficiency. For the same reason, an Elastosil\textsuperscript{\textregistered} RT 604 silicone pad is used to couple the scintillators to the SiPM array. This optical coupling pad is separated by a white PLA\footnote{Polylactic acid} grid reducing the amount of optical crosstalk between the pixels. In Figure \ref{fig:detector_setup}, photographs of the detector components are shown. 

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.30\textwidth}
    \includegraphics[width=\textwidth]{Detector/photo_detector16px.jpg}
    \subcaption{Scintillator matrix}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
    \includegraphics[width=\textwidth]{Detector/sipmarray_cut.jpg}
    \subcaption{SiPM array}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
    \includegraphics[width=\textwidth]{Detector/20200709_101846.jpg}
    \subcaption{Optical coupling pad}
    \end{subfigure}
    \caption{Photographs of the $4\times4$ pixel detector components.}
    \label{fig:detector_setup}
\end{figure}


\subsubsection{Stilbene}
The usage of the organic scintillator crystal stilbene (chemical formula \ce{C14H12}) enables the discrimination of neutron- and gamma-induced signals. For gamma interactions, the scintillation light is created by electrons while for neutron interactions, the scintillation light mainly comes from proton recoil events. Stilbene shows longer decay times of scintillation light emission for neutron-induced signals, than for gamma-induced signals \cite{stilbene_decay}. Therefore, neutron-induced signals have a longer falling edge, allowing neutron-gamma discrimination by pulse shape discrimination methods. \\
Stilbene shows a significant quenching effect. The same amount of deposited energy leads to much fewer scintillation light when caused by heavy charged particles (e.g. protons) instead of electrons. For electrons, a linear relation between the deposited energy and the scintillation light output can be assumed, while the relation is non-linear for heavy charged particles \cite{stilbene_quenching_1, stilbene_quenching_2}. Also, an anisotropy of Stilbene's light response for proton recoils is reported, depending on the direction of the recoil relative to the crystal axes \cite{anisotropy}.

%\subsubsection{SiPMs}
\subsubsection{Electronics}
The detector readout system is shown as a schematic sketch in Figure \ref{subfig:blockdiagram}. It consists of the SiPM array plus the front end custom electronics board developed in-house, and the digitization system. \\
The front end electronics board includes the amplifier circuits for all 16 SiPM channels as well as the SiPM power supplies. For each channel, a positive and a negative unipolar output signal is provided to enable the use of different digitizer types. For the SiPM power supply, two Hamamatsu MPPC\textsuperscript{\textregistered} C11204-02 slow control chips \cite{HamamatsuPS} are used. This chip allows for a temperature correction of the SiPM's bias voltage in order to keep the SiPM gain constant. Figure \ref{subfig:camerasetup} shows a photograph of the $4 \times 4 $ detector mounted on the front end electronics board. The detector and the board are placed inside an aluminium box. \\
For signal digitization, two CAEN N6730B FADCs \cite{CAENFADC} are used. They have a sampling rate of up to \SI{500}{MS \per \second}, a resolution of 14 bits and a dynamic range of \SI{2}{Vpp}.

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.47\textwidth}
    \includegraphics[width=1.\textwidth]{Detector/blockschaltbild.png}
    \subcaption{}
    \label{subfig:blockdiagram}
    \end{subfigure}
    \begin{subfigure}{0.47\textwidth}{
    \includegraphics[width=1.\textwidth]{Detector/camera_setup.png}
    \subcaption{}
    \label{subfig:camerasetup}
    }
    \end{subfigure}
    \caption{(a): Schematic sketch of the detector readout. (b): Photograph of the $4 \times 4$ detector with its front end electronics.}
    \label{fig:electronics_setup}
\end{figure}

\subsection{Pulse Shape Discrimination}
\label{sec:psd}
The classification of signals as neutron- or gamma-induced is based on the Tail-to-Total pulse shape discrimination (PSD) method. All analyses described in the following are done individually for each detector pixel. \\
In a first instance, the recorded signals are baseline-corrected and pile-up events and microwave-induced portions of the signal (caused by the neutron generator ion source) are filtered. For each remaining event, a PSD variable is calculated that is defined as the ratio of the tail integral $Q_\mathrm{Tail}$ and the total integral of the pulse $Q_\mathrm{L}$:
\begin{equation}
    PSD = \frac{Q_\mathrm{Tail}}{Q_\mathrm{L}} = \frac{Q_\mathrm{L}-Q_\mathrm{S}}{Q_\mathrm{L}}
\end{equation}
$Q_\mathrm{Tail}$ can also be expressed using $Q_\mathrm{L}$ and the short integral $Q_\mathrm{S}$ over the beginning of the pulse. The integrals are defined relative to the \textit{trigger position}, $t_\mathrm{Trg}$, where $50\%$ of the pulse height is reached, and are given by
\begin{equation}
    Q_\mathrm{L,S} = \int_{t_\mathrm{Trg} + \Delta_\mathrm{off}}^{t_\mathrm{Trg} + \Delta_\mathrm{L,S}}{S(t)\mathrm{d}t}
\end{equation}
with the signal $S(t)$. The integration limits were optimized with regard to the neutron-gamma separation to $\Delta_\mathrm{off} = -40\,\si{\nano\second}$, $\Delta_\mathrm{S} = 24\,\si{\nano\second}$ and $\Delta_\mathrm{L} = 270\,\si{\nano\second}$.  

\subsubsection{Energy calibration}
An energy calibration was performed to translate the pulse integral in $\mathrm{mV \cdot ns}$ into the energy deposited in $\mathrm{keV}$ electron equivalent ($\mathrm{keVee}$). For the calibration, a \isotope[22]{Na} and a \isotope[207]{Bi} radioactive source were used. The calibration was done using the compton edge position, as no photopeak is visible in the recorded gamma spectra due to the low atomic number of the elements present. The position is determined following the procedure described in \cite{calibration}. A linear relation between the pulse integral and deposited energy is assumed, based on a fit to the four measured calibration compton edge energies and their corresponding pulse integrals. 

\subsubsection{Neutron-gamma classification and particle detection rate}
When creating a 2D histogram with the energy in $\mathrm{keVee}$ on the x-axis and the PSD variable on the y-axis, a plot with two distinct bands is created. An example plot is shown in Figure \ref{fig:psd_3sigma}. The upper band can be assigned to neutron events (``neutron band''), the lower band to gamma events (``gamma band''). \\
To quantify the amount of neutron and gamma events, 1D histograms of the PSD variable can be produced over the range of energies over a given bin width, corresponding to vertical slices from the 2D histogram. If neutron and gamma events are separated, within such a 1D histogram, two peaks form which can be described by a double-Gaussian fit. The peak region at lower PSD corresponds to gamma events and the other one to neutron events. For higher energies, almost no events occur in the neutron band region. Therefore, only the gamma band is fitted in this region. From the fit results, the neutron and gamma band limits are calculated as the $3\sigma$ boundaries of the Gaussians at each energy. These boundaries can then be portrayed as lines on the 2D histogram. In Figure \ref{fig:psd_3sigma}, the $3\sigma$ boundaries of both bands are shown as green and red lines. Here, the neutron band limits are extrapolated horizontally into the energy region where almost no neutron events occur. 
A criterion for the separation is the \textit{Figure of Merit (FOM)}:
\begin{equation}
    FOM = \frac{\mu_n - \mu_g}{FWHM_n + FWHM_g} = \frac{\mu_n - \mu_g}{2\sqrt{2 \ln(2)}(\sigma_n + \sigma_g)}
    \label{eq:FOM}
\end{equation}
In case the separation is exactly $3(\sigma_n + \sigma_g)$, the formula simplifies to $FOM = \frac{3}{2\sqrt{2 \ln(2)}}  \approx 1.27$. When calculating the FOM for all slices, one can see that it increases towards higher energies, exceeding the $3\sigma$ separation value of $FOM=1.27$. In Figure \ref{fig:psd_3sigma}, the energy where $FOM=1.27$ is exceeded is marked as red dashed line. For the region to the right of the $FOM=1.27$ position, an event is classified as neutron (gamma) if it lies inside the $3\sigma$ region of the neutron (gamma) band. The region to the left of the $FOM=1.27$ position is not taken into account as sometimes fit problems occur and the determined event type separation would be highly dependent on the chosen fitting parameters. \\ 
The accepted neutron and gamma rates are calculated from the particle counts in the acceptance regions divided by the measurement time. The rates differ from pixel to pixel, typical values for neutrons lie around $10\,\mathrm{Hz}$ for the measurements described in this paper. For the example shown in Figure \ref{fig:psd_3sigma}, the accepted neutron rate is $(11.06 \pm 0.06)\,\si{\Hz}$, corresponding to $2.2\%$ of the recorded events. The accepted gamma rate is $(3.57 \pm 0.03)\,\si{\Hz}$, corresponding to $0.7\%$ of the events. Most of the other recorded events lie at very low pulse integrals where no reliable separation between gammas and neutrons can be determined. \\
The $3\sigma$ limits described above are always determined for measurements without any object in front of the detector. In case additional measurements with objects are done with the same detector settings, the limits are re-used and applied to these measurements. The reason is that the absorption measurements are always put in relation to the measurement without object (the so-called calibration image), see also section \ref{subsec:Absorption_meas}.

\begin{figure}[htbp!]
\centering
\begin{subfigure}{.67\textwidth}
\includegraphics[width=\textwidth]{PSD/fitbands_cal_pixelA4_forward_noAbs.png}
\end{subfigure}
~
\begin{subfigure}{.31\textwidth}
\includegraphics[width=\textwidth]{Detector/pixel_labeling.pdf}
\end{subfigure}
\caption{Left: Example PSD plot, detector pixel A4. The $3\sigma$ limits of the neutron and gamma band are shown in green and red. Extrapolations are performed to the regions where too few events for Gaussian fits are located. The red dashed line marks the energy where $FOM=1.27$. Right: Detector pixel labeling, as seen from the incoming particle's perspective.}
\label{fig:psd_3sigma}
\end{figure}



%\begin{figure}[h!]
%    \centering
%    \begin{subfigure}{0.47\textwidth}
%    \includegraphics[width=\textwidth]{PSD/scatterplot_keVee_pxA4_nonlog.png}
%    \subcaption{}
%    \label{subfig:psd_3sigma}
%    \end{subfigure}
%    \begin{subfigure}{0.47\textwidth}
%    \subcaption{}
%    \label{subfig:psd_projection}
%    \end{subfigure}
%    \caption{In (a): Analyzed PSD plot. The $3\sigma$-environments of the neutron and gamma band are shown in green and red. Extrapolations are performed to the regions where too few events for gaussian fits are located. The red dotted line marks the energy where $FOM=1.27$. In (b): Exemplary projection to the PSD axis for an energy slice in between ...and ... In red, the double gaussian fit is shown.}
%    \label{fig:PSD_analyzed}
%\end{figure}



==> geant4.tex <==
\subsection{Comparison with Geant4 simulations}
\label{sec:Geant4}
Geant4 simulations of the setup were done to better understand the neutron interactions in the attenuator objects and in the detector. 

\subsubsection{Geant4 setup}
The Geant4 simulation setup consists of a detailed detector model along with attenuator objects and optionally a PE block, as shown in Figure \ref{fig:geant4model}.
It is assumed that incoming neutrons are emitted from a point source at \SI{80}{cm} distance from the detector with spectrum defined according to an emission in either the forward or \SI{90}{\degree} direction. \\
The simulation stores the neutron interactions in the step wedge and the interactions, energy losses by particle type and amount of created scintillation light in the detector pixels. 
Geant4 version 10.05.p01 \cite{Geant4} is used, the physics list essentially corresponds to the QGSP\textunderscore BIC\textunderscore HP list, but using G4EmStandardPhysics\textunderscore option4 and G4OpticalPhysics \cite{Geant4Physics}. The JEFF3.3 library is used for the neutron interaction data. The particle-dependent scintillation light output is modeled based on Birk's law \cite{Birk}. 

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.7\textwidth]{Geant4/Example_stepwedge_rotated_3_labels.png}
    \caption{Geant4 detector model with attenuator step wedge (Fe-Al-PMMA) placed in front of the detector. In the simulation, steel is approximated as pure iron because the exact steel composition is unknown, but the difference in attenuation should be very small.}
    \label{fig:geant4model}
\end{figure}

\subsubsection{Spectra and Efficiency}
One aspect of the simulation is the amount of scintillation light, which can be transferred to an energy spectrum in keVee by dividing the number of photons by stilbene's light yield. When excluding scintillation light caused by electrons and gammas, one gets a spectrum that can be compared to the measured one. In Figure \ref{fig:sim_spec}, very good agreement between simulation and experiment can be seen for two different pixels. In order to achieve this agreement, the simulation parameters \textit{Birk's constant, kB,} and the \textit{intrinsic resolution} were optimized. A larger value of $kB$ means that proton recoils lead to less light compared to electron interactions. The intrinsic resolution describes the fluctuation of the amount of created scintillation light. It turned out that to get a good agreement for most pixels at least two different classes of stilbene need to be defined, one with a Birk's constant of $kB=0.135~\si{mm/MeV}$ and one with $kB=0.185~\si{mm/MeV}$ (red or blue stilbene crystals in Figure \ref{fig:geant4model}). These values of $kB$ cannot be seen as a physical Birk's constant but are simply parameters used to increase the simulation accuracy. The same is true for the intrinsic resolution. A reason for the pixel to pixel differences may be the anisotropy of stilbene \cite{anisotropy}, but also differences in the light propagation within the scintillators and the light detection at the SiPMs could play a role. This light propagation is not included explicitly in the simulation, so its effect is instead represented by the tuning of these parameters. 

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=.45\textwidth]{Geant4/comparespec_sim_A1_180820.png}
    \quad
    \includegraphics[width=.45\textwidth]{Geant4/comparespec_sim_B1_180820.png}
    \caption{Example simulated (black) and measured (green) spectra, representing the two different stilbene classes. The red and blue dashed lines mark the experimental FOM=1.27 position and the artificial energy cut at \SI{450}{keVee}.  Left: Pixel A1. Right: Pixel B1. The energies are significantly smaller than for pixel A1.}
    \label{fig:sim_spec}
\end{figure}

\noindent To calculate the simulated detection efficiency, the experimentally determined $FOM=1.27$ values are applied to the spectra pixel per pixel and the integral of the remaining spectra is calculated. Also, a simulation with a PE block was performed and its resulting spectrum subtracted. By dividing by the expected incoming neutron rate at the detector, the efficiency is obtained. For the optimized simulation setup, a mean detection efficiency of $(9.87 \pm 0.01)\%$ in the forward direction was determined. This is approximately $0.3$ percentage points higher than the experimentally determined value and compatible with this result within the overall experimental uncertainty. When applying a \SI{450}{keVee} threshold instead of the $FOM=1.27$ thresholds to the simulated data, the mean efficiency is with $(6.25\pm0.01)\%$ approximately 0.9 percentage points larger than the experimental value.\\
In the \SI{90}{\degree} direction, however, the simulated efficiency is only $(9.36 \pm 0.01)\% $, so approximately 2.5 percentage points smaller than the experimental one, and particularly smaller than in the forward direction. One reason for the higher experimental efficiency is the behavior of pixels A2 and A3, where the experimental efficiencies have quite large uncertainties compared to the other pixels, while the simulation uncertainties are similar for all pixels. This influences the weighted mean efficiency. However, also for the other pixels, the simulated efficiencies are around 1.5-2 percentage points smaller. When applying the \SI{450}{keVee} threshold instead, the mean efficiency is $(4.70\pm0.01)\%$, which is very close to the experimental result. It is therefore still an open question where the discrepancy for the FOM criterion comes from. Also, to get a good agreement between the simulated and measured spectra, the values of the $kB$ parameters need to be set to \SI{0.125}{mm/MeV} and \SI{0.175}{mm/MeV}, indicating a tendency to larger pulse heights at the same amount of deposited energy than for the forward direction measurement. It is an open question what causes these differences. It could be a temperature effect in the measurements, e.g. a higher SiPM overvoltage, even though a temperature correction is applied to the SiPM bias voltage. The SiPM temperature during the \SI{90}{\degree} measurements was approximately \SI{2}{\celsius} lower than during the forward direction measurements. 

\subsubsection{Simulated images and macroscopic cross section}
Figure \ref{fig:sim_mac} shows the simulated macroscopic cross section $\Sigma$ determined from a simulation with the Fe-Al-PMMA step wedge which assumes a perfect alignment of the step wedge in front of the pixels and the detectors with respect to the source. The determination method of $\Sigma$ is similar to the experiment. \\
As in the experiment, the calculated cross sections are significantly smaller than the literature values for all three materials. Two possible reasons were identified in the simulation. The first contribution is from neutrons interacting in both the object and the detector, which cause up to approximately 8\% of the detected neutrons in the simulation. It is seen in the simulation that this effect alone cannot fully describe the discrepancy between simulated and literature cross sections. Another contribution could come from multiple interactions in the detector, either in two or more different pixels or in the detector housing and then in a pixel, leading to a background rate of neutrons. The background generated in this way reduces the determined cross section and is of relatively greater importance for pixels covered with a higher-attenuating material and/or a greater material thickness. This effect is not corrected by subtracting the PE measurement, as the PE block is much larger than the detector volume. Multiple interaction events in detector pixels with at least one interaction above the required FOM threshold occur in about 20\% - 25\% of the simulated events when assuming the mean FOM threshold of \SI{318}{keVee} in the forward direction. However, this value also includes very small energy losses of a few keV and does not consider if the neutron was scattered into the pixel where it was detected or vice versa. Using e.g. an arbitrarily chosen \SI{100}{keV} threshold, which corresponds to approximately 3.5\% of the initial neutron energy, the multi-pixel interaction fraction already reduces to approximately 13\%.  Additionally, neutrons that interact in the detector box and then in the detector need to be considered. It would be interesting for the future to extend the simulation so that neutrons that interact first somewhere in the detector box or e.g. in an uncovered pixel and then in a certain covered pixel are counted to quantify the influence on the determined macroscopic cross section.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=.7\textwidth]{Geant4/simulated_Sigma_forward115kV.pdf}
    \caption{Simulated macroscopic cross section determined from the Fe-Al-PMMA step wedge's neutron attenuation. The literature cross sections are added for comparison as dotted lines.}
    \label{fig:sim_mac}
\end{figure}

\noindent The decrease of the cross section towards higher material thicknesses is smaller in the simulation than in the experiment. Also, the simulated cross sections for small material thicknesses seem to be smaller than in the experiment. A possible explanation could be a slight misalignment of the step wedge in the experiment. This could either be a shift or a rotation of the step wedge compared to the direct neutron direction of flight. To investigate effects of shifts, the step wedge in the simulation was misaligned in the vertical and horizontal direction by $\pm 1~\si{mm}$ and $\pm~2 \si{mm}$. It should be mentioned that a \SI{2}{mm} shift in the experiment is quite unlikely as great effort was made to correctly position the step wedge in front of the detector. \\
A misalignment in horizontal direction to the right, shifting the PMMA part slightly into the empty detector row can be limited to (much) less than \SI{1}{\milli\meter} as this misalignment would cause a much larger shadowing of up to approximately $-12\%$ in the empty row than observed in the measurement. Also, a shift of \SI{2}{mm} to the left can be excluded, as this would cause a smaller experimental cross section for PMMA than for Al, which is also not observed.
The decrease of the cross section towards higher material thicknesses could be i.a.~explained by a shift upwards. In this case, a pixel e.g. covered with \SI{1}{cm} of material would also be partially covered by \SI{2}{cm} of material, leading to a higher cross section. This effect is as a percent larger for the small material thicknesses. A simulation with such a shift of \SI{1}{mm} fits better to the data than the unshifted simulation. To illustrate this, correction factors for the cross section can be calculated from the simulated data by dividing the literature macroscopic cross sections by the simulated ones. When multiplying the experimental values by the correction factor, the resulting values should ideally correspond to the literature cross sections. Figure \ref{fig:corrected_xs} shows the results for the original and the vertically shifted case. The shifted simulation leads to better agreement between corrected values and literature values, even though there are still some deviations (e.g. \SI{6}{cm} of PMMA). However, it can be concluded that lower experimental macroscopic cross sections are expected, and the exact dependency of the thickness is probably explained by alignment difficulties.

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}{.47\textwidth}
    \includegraphics[width=\textwidth]{Geant4/fGraph_mac_corr_noshift.png}
    \subcaption{No shift.}
    \end{subfigure}
    \begin{subfigure}{.47\textwidth}
    \includegraphics[width=\textwidth]{Geant4/fGraph_mac_corr.png}
    \subcaption{Vertical shift by \SI{1}{mm}.}
    \end{subfigure}
    \caption{Corrected experimental macroscopic cross sections by the simulated cross sections. (a): Using data from the unshifted simulation. (b): Using data from the vertically shifted simulation by \SI{1}{mm} upwards. }
    \label{fig:corrected_xs}
\end{figure}

==> measurement_setup.tex <==
As mentioned above, measurements at three different angles relative to the ion beam path line, i.e. three different mean initial neutron energies, were performed. In Table \ref{tab:measurement_positions}, the angles and the corresponding mean neutron energies are given. \\
Photographs of the measurement setup are shown in Figure \ref{fig:setup}. The detector is positioned on an aluminium plate at a distance of approximately \SI{80}{\centi\metre} away from the neutron emission spot. The exact distances are listed in Table \ref{tab:measurement_positions}. A sample holder is attached to the detector to be able to position small absorber objects in front of the detector. The objects are further described in section \ref{subsec:Absorption_meas}. A lead plate of approximately 1-2 \si{\milli\metre} thickness is placed around the neutron generator to shield low-energetic X-rays. There is also the possibility to place a polyethylene (PE) block of size $21 \times 10 \times 5.5~\si{cm^3}$ in between the generator and the detector to determine the neutron background. The PE block is expected to shield more than $99.5\%$ of the neutrons directly coming from the generator. The remaining detected neutrons are therefore assumed as ``background'' neutrons which did not travel directly from source to detector, but rather scattered off of the floor, ceiling, walls, etc. Measurement times per configuration setup varied between approximately \SI{0.5}{h} and \SI{1}{h}.

\begin{table}[htbp!]
    \centering
    \caption{Measurement positions and corresponding mean neutron energies. The angle is relative to the ion beam path line. The distances are determined from the neutron emission spot to the scintillators' front surface positions.}
    \label{tab:measurement_positions}
    \begin{tabular}{c|c|c}
        Angle & Mean $E_\mathrm{n}$ [MeV] & Distance [cm] \\
        \hline
        \SI{0}{\degree} & 2.84 & $81.0 \pm 2.0$ \\
        \SI{90}{\degree} & 2.47 & $81.8 \pm 2.0$ \\
        \SI{115}{\degree} & 2.33 & $79.4 \pm 2.0$ 
    \end{tabular}
\end{table}

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}{.49\textwidth}
    \includegraphics[width=\textwidth]{Generator_Nina/setup_fw_PE_labels.png}
    \subcaption{}
    \end{subfigure}
    ~
    \begin{subfigure}{.49\textwidth}
    \includegraphics[width=\textwidth]{Generator_Nina/detector_stepwedge_labeled.png}
    \subcaption{}
    \end{subfigure}
    \caption{Photographs of the measurement setup (in forward direction). (a): Overview. (b): Detector and absorber sample.  \textit{   (*) PE block only used for background measurements}.}
    \label{fig:setup}
\end{figure}

==> results.tex <==
In the following, selected measurement results obtained with the D-D generator setup are presented. A determination of the detection efficiency for D-D neutrons is presented and discussed. Furthermore, neutron absorption images of different objects are evaluated.

\subsection{Detection efficiency for D-D neutrons}
The detection efficiency $\epsilon$ is defined by 
\begin{equation}
    \epsilon = \frac{R_\mathrm{det}}{R_\mathrm{inc}}
\end{equation}
with the detected neutron rate $R_\mathrm{det}$ and the incoming neutron rate at the scintillator position $R_\mathrm{inc}$, which can be expressed by 
\begin{equation}
    R_\mathrm{inc} = R_0 \cdot \frac{F_\mathrm{det} \cdot f_\mathrm{geom} \cdot f_\mathrm{abs} }{4 \pi d^2}
\end{equation}
Here, $R_0$ is the emitted neutron rate, $d$ is the distance to the detector and $F_\mathrm{det}$ is the scintillators' front surface area. The factor $f_\mathrm{geom}$ describes the non-isotropic neutron emission of the generator, see also section \ref{sec:generator}. The factor $f_\mathrm{abs}$ describes the attenuation of neutrons in the generator itself or in the lead plate used to shield X-rays. For the estimation of $f_\mathrm{abs}$, microscopic cross section data from the JEFF 3.3 \cite{JEFF} and ENDF/B-VII.1 \cite{ENDF} database evaluated for the neutron generator output spectrum is used. An uncertainty of 2\% is assumed, due to uncertainties on the lead plate thickness, the cross sections and the neutron paths through the generator.
For the detected rate $R_\mathrm{det}$, two measurements are necessary. First, a measurement without any object between the generator and the detector, which includes detected neutrons both directly from the generator and scattered from other directions (background neutrons). For the efficiency calculation, only the direct neutrons are needed. Therefore, the background rate $R_\mathrm{BG}$ needs to be subtracted. The background is determined from a measurement with PE block, as described in section \ref{subsec:setup}. The neutron rate from this measurement must be weighted by the neutron generator output during the efficiency measurement, as the output varies with time.

\subsubsection{Uncertainty estimation}
The uncertainty on the efficiency consists of two parts: a statistical uncertainty from the particle counts that varies from detector pixel to pixel, and a correlated systematic uncertainty for all pixels due to the incoming neutron rate. This systematic uncertainty would shift all efficiencies in the same direction.\\
The statistical uncertainty can be subdivided into a Poisson error based on the number of counts as well as an uncertainty from the $FOM=1.27$ position. The main contributions to the systematic uncertainty are the errors on the initial neutron rate $R_0$, on the distance $d$ and on the factor $f_\mathrm{abs}$. The errors are propagated to $\epsilon$ via Gaussian error propagation. \\
The weighted mean over all pixels is calculated taking only the statistical uncertainties into account. To illustrate the effect of the correlated uncertainty, the weighted mean is also calculated after shifting the data by $1\sigma_\mathrm{sys}$ up or down.


\subsubsection{Results}
In Figure \ref{fig:efficiency_forward}, the detection efficiencies for each pixel determined from a measurement in the forward direction are shown. In Figure \ref{fig:efficiency_90and115deg}, the same is shown for measurements along the \SI{90}{\degree} and the \SI{115}{\degree} directions. \\
The efficiency lies overall in the order of $10\%$, but fluctuates from pixel to pixel. Especially pixel A3 has a much smaller efficiency than the other pixels in all measurements. A closer look at this pixel shows that its pulses are smaller and the separation between neutrons and gammas is worse than for most other pixels. In contrast, the pixels B2, C4, and D4 show an above average efficiency. In these pixels the neutron band ends at relatively high energy combined with good particle separation. The fluctuations from pixel to pixel may be explained by setup differences such as the coupling qualities between the scintillators and the SiPMs, or by differences of the crystals themselves. Differences can occur in light propagation (e.g., different surface structures), but also in scintillation light creation, e.g., due to Stilbene's anisotropy \cite{anisotropy}.  \\
When comparing the forward direction with the \SI{90}{\degree} and \SI{115}{\degree} direction, it is seen that the efficiency in \SI{90}{\degree} direction seems to be approximately 2.4 percentage points larger, while in \SI{115}{\degree} direction, the efficiency is slightly smaller. The variation from pixel to pixel however looks similar in all measurements. A larger efficiency in \SI{90}{\degree} direction is a priori unexpected, as the neutron energy is smaller and therefore the number of events above the energy threshold should be smaller. This effect should only be slightly compensated by the higher proton recoil interaction cross section in stilbene at around \SI{2.45}{MeV}. The difference is probably not explained by the uncertainty in the total neutron generator output, as this error corresponds to a shift of the output that should be in the same direction for all measurements. Also, the uncertainty on the distance and the self-absorption cannot explain the large difference. We therefore think that the reason lies within the way the signal data was processed, in terms of what signals are considered neutron events and which not. As described in section \ref{sec:psd}, only the $FOM>1.27$ energy region in the PSD plot is considered for neutron counting, and this is determined separately for each angle. For the \SI{90}{\degree} measurement, $FOM=1.27$ is reached at $E=303.2\,\si{keVee}$ when averaging over all pixels, for the forward direction, it is reached at $E=318.7\,\si{keVee}$, indicating a better separation of neutron and gamma band in \SI{90}{\degree} direction. The lower threshold needed to achieve the defined $FOM$ leads to a larger energy range that is considered for the neutron counting, and effectively a higher detection efficiency. When applying an arbitrarily chosen constant higher energy threshold of \SI{450}{keVee} across all measured data, which is slightly above the largest $FOM=1.27$ position, the mean efficiency in the \SI{90}{\degree} direction is $4.7\,\%$, which is smaller than the forward direction value of $5.4\,\%$, which fits qualitatively much better to the expected trend. One possible explanation for the variation in neutron to gamma separation is a varying amount of gamma flux around the source, for example if one direction was better shielded with lead than another. The lead shielding was not applied in a precisely uniform way, and that might contribute to this effect and the variation in efficiency from one direction to another. This effect might be even stronger if X-rays (not gammas) are contributing to the ``gamma'' contribution, as they are more sensitive to variations in the lead shielding. Even though they are nominally of too-low energy to be registered as gamma events, it might be that a very small percentage of them interact within the stilbene very close to the surface of the SiPM, and therefore produce an abnormally large signal which appears as a relatively high energy.  However, to be certain this should be studied more carefully in the future.

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=\textwidth]{Efficiency/PSI_DD_AbsStair_fw_7_02032020_plot_efficiency_PE_corr_avshift_pb1_5mm.pdf}
    \caption{Detection efficiency in \SI{0}{\degree} direction for each detector pixel. Three uncertainties are shown. The statistical (Poisson) uncertainty due to the particle counts (in black), an uncertainty due to the error on the $FOM = 1.27$ position (in blue) and a combined uncertainty including the systematic error arising from the error on $R_\mathrm{inc}$ (in green). Also, the weighted mean (green line) with its statistical and systematic error (green dotted lines) is shown. }
    \label{fig:efficiency_forward}
\end{figure}

\begin{figure}[htbp!]
\centering
\begin{subfigure}{.47\textwidth}
\includegraphics[width=\textwidth]{Efficiency/PSI_DD_NoAbs90Deg_AbsStair_fw_2_03032020_plot_efficiency_PE_corr_avshift_pb1_5mm.pdf}
\subcaption{\SI{90}{\degree} direction}
\end{subfigure}
\begin{subfigure}{.47\textwidth}
\includegraphics[width=\textwidth]{Efficiency/PSI_DD_AbsStair115Deg_fw_5_03032020_plot_efficiency_PE_corr_avshift_pb1_5mm.pdf}
\subcaption{\SI{115}{\degree} direction \textit{(*)}}
\end{subfigure}
\caption{Detection efficiency in \SI{90}{\degree} and \SI{115}{\degree} direction for each detector pixel. For an uncertainty description, see Figure \ref{fig:efficiency_forward}. \textit{(*): No data for pixel C4 available as it wasn't connected to the readout electronics in this measurement. }}
\label{fig:efficiency_90and115deg}
\end{figure}




\subsection{Attenuation measurements}
\label{subsec:Absorption_meas}
The goal of the attenuation measurements is the experimental measurement of fast neutron attenuation in different materials, leading to the calculation of the macroscopic cross section and its comparison to literature values. The attenuation of gammas is not considered, as the neutron generator does not produce initial gammas but they are rather created from activation processes in all surrounding materials, so that their direction of origin is unknown. The recorded gamma interactions are rejected by pulse shape discrimination. \\
Three different attenuation objects (see Figure \ref{fig:absorbers}) are investigated by placing them on a sample holder directly in front of the detector. The detector is placed in the forward direction relative to the generator. 
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=.7\textwidth]{Absorber/absorbertreppen.jpg}
    \caption{Photograph of the absorber objects. Left and mid: Small step wedges, step sizes $\{0.5,1.0,1.5,2.0\}\,\si{cm}$. The material combinations are Al-PMMA and PVC-Steel. Right: Large step wedge with step sizes $\{1,2,4,6\}\,\si{cm}$. The materials are steel, Al, PMMA.}
    \label{fig:absorbers}
\end{figure}

\noindent To determine the attenuation of an object, three measurements (images) must be taken: a so-called calibration image without any material placed in front of the camera, the so-called absorption image with the object and a background image with the PE block. In each case, a neutron rate $R_i$ with $i \in \{cal, obj, BG\}$ relative to the incoming neutron rate is calculated. The neutron attenuation can then be expressed by the \textit{differential rate} ($\Delta Rate$) that can be defined as 

\begin{equation}
    \label{eq:DeltaRate}
    \Delta Rate = \frac{(R_\mathrm{obj} - R_\mathrm{PE}) - (R_\mathrm{cal} - R_\mathrm{PE})}{R_\mathrm{cal} - R_\mathrm{PE}} = \frac{R_\mathrm{obj} - R_\mathrm{PE}}{R_\mathrm{cal} - R_\mathrm{PE}} -1
\end{equation}

\noindent From the differential rate, the macroscopic cross section $\Sigma$ can be calculated by

\begin{equation}
   \label{eq:attenation_exp}
   R_\mathrm{obj} - R_\mathrm{PE} = (R_\mathrm{cal} - R_\mathrm{PE})\cdot e^{-\Sigma \cdot x} 
\end{equation}

\begin{equation}
    \label{eq:Sigma_exp}
     \Sigma = \frac{-1}{x} \ln{\left( \frac{R_\mathrm{obj} - R_\mathrm{PE}}{R_\mathrm{cal} - R_\mathrm{PE}}\right)} = \frac{-1}{x} \ln{\left(\Delta Rate +1\right)}
\end{equation}
The uncertainties of $\Delta Rate$ and $\Sigma$ are calculated via Gaussian error propagation from the uncertainties of $R_i$. Since the detector is not moved during a given measurement series, the uncertainties related to the detector position do not need to be considered. 

\subsubsection{Results}
Figure \ref{fig:diffrate} shows the differential rates for the large step wedge and the small Al-PMMA\footnote{Polymethyl methacrylate} and PVC-Steel step wedges (photo in Figure \ref{fig:absorbers}). 
The large step wedge covers the detector pixel columns 1, 2 and 3 with steel, aluminium and PMMA. The pixel column 4 is left uncovered. The pixel row A is covered with \SI{6}{\centi \metre} of material, B with \SI{4}{\centi \metre}, C with \SI{2}{\centi \metre} and D with \SI{1}{\centi \metre} (for detector pixel arrangement, see Figure \ref{fig:psd_3sigma}). Looking at the differential rates, one can clearly identify the steps of the step wedge. Also, differences between the materials can be seen. The smallest attenuation is seen for \SI{1}{\centi\metre} aluminium, the largest attenuation for  \SI{6}{\centi \metre} steel. Overall, aluminium is the weakest attenuator, steel the strongest. For the uncovered row, no significant rate reduction is seen, indicating especially no shadowing effect. \\
The small step wedges cover all detector pixels. Always two neighbouring pixels are covered by the same material thickness. The pixel columns 1 and 2 are covered with Al (PVC), the columns 3 and 4 with PMMA (steel). Pixel rows C and D are covered by \SI{0.5}{\centi \meter} or  \SI{1.5}{\centi \meter}, A and B by  \SI{1}{\centi \metre} or  \SI{2}{\centi \metre} of material. In the differential rates, these small thickness differences are still visible, despite some fluctuations. As for the large step wedge, aluminium is the weakest attenuator, it absorbs less than PMMA and slightly less than PVC. The strongest attenuator is Steel. However, the differential rates also show a characteristic problem of the radiographic imaging method. For example, $\Delta Rate$ for \SI{1.5}{\centi \meter} Al and \SI{1}{\centi \meter} PMMA are comparable, so, for an unknown sample, it would be impossible to discriminate between two such objects in case both material and thickness are unknown. If one or the other is known a priori, then the other can potentially be determined from a radiographic image, as long as the materials to be identified have sufficiently different attenuation coefficients. With a tomographic image, this problem is not present, and a spatial distribution of the attenuation coefficient could be determined.  

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}{.47\textwidth}
    \includegraphics[width=\textwidth]{Absorber/diffrate_stepwedge.png}
    \subcaption{}
    \end{subfigure}
    \begin{subfigure}{.47\textwidth}
    \includegraphics[width=\textwidth]{Absorber/diffrate_stepwedge_AlPMMA_PVCFe.png}
    \subcaption{}
    \end{subfigure}
    \caption{Measured neutron differential rates for the step wedges. (a): Steel-Al-PMMA step wedge. Materials from left to right: Steel $\{6,4,2,1\}\,\si{\centi\meter}$, Al $\{6,4,2,1\}\,\si{\centi\meter}$, PMMA $\{6,4,2,1\}\,\si{\centi\meter}$, not-covered. (b): Al-PMMA and PVC-Steel step wedge. Materials from left to right: Al (PVC) $\{1,1,0.5,0.5\}\,\si{\centi\meter}$, Al (PVC) $\{2,2,1.5,1.5\}\,\si{\centi\meter}$, PMMA (Steel) $\{2,2,1.5,1.5\}\,\si{\centi\meter}$, PMMA (Steel) $\{1,1,0.5,0.5\}\,\si{\centi\meter}$.}
    \label{fig:diffrate}
\end{figure}

\noindent From the $\Delta Rates$, the macroscopic cross sections are calculated according to equation \eqref{eq:Sigma_exp}. The resulting values are shown in Figure \ref{fig:mac_crosssection} both for the large step wedge  and the small step wedges Al-PMMA and PVC-Steel. The figures also show the theoretically expected values according to literature microscopic cross section data (JEFF3.3 and ENDF/B-VII.1 database) combined with the previously given fast neutron spectra. It can be seen that the experimentally determined cross sections are generally significantly smaller than the literature values. For the large step wedge, the difference gets larger as the material thickness increases, especially for steel. However, the relative attenuation from one material to another qualitatively follows the expected trend. This discrepancy was further studied using simulations, as described in section \ref{sec:Geant4}. The results from the large and the small step wedges for steel, Al and PMMA are within the uncertainties. The material sequence is correctly reproduced within the uncertainties.

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}{.47\textwidth}
    \includegraphics[width=\textwidth]{Absorber/PSI_DD_AbsStair_fw_7_02032020_Sigma_PE.pdf}
    \subcaption{Step wedge Steel-Al-PMMA}
    \end{subfigure}
    \begin{subfigure}{.47\textwidth}
    \includegraphics[width=\textwidth]{Absorber/PSI_DD_AbsSmallStep_fw_10_02032020_Sigma_PE.pdf}
    \subcaption{Step wedges Al-PMMA and PVC-Steel}
    \end{subfigure}
    \caption{Macroscopic cross section for steel, aluminium, PMMA, and PVC, determined from measurements with the Fe-Al-PMMA step wedge (in (a)) and the small step wedges (in (b)). The literature values calculated from JEFF 3.3 and ENDF/B-VII.1 microscopic cross section data are marked in the plots as dotted lines.  }
    \label{fig:mac_crosssection}
\end{figure}



